Maximum Likelihood Estimation for Learning Populations of Parameters

Consider a setting with $N$ independent individuals, each with an unknown parameter, $p_i \in [0, 1]$ drawn from some unknown distribution $P^\star$. After observing the outcomes of $t$ independent Bernoulli trials, i.e., $X_i \sim \text{Binomial}(t, p_i)$ per individual, our objective is to accurately estimate $P^\star$. This problem arises in numerous domains, including the social sciences, psychology, health-care, and biology, where the size of the population under study is usually large while the number of observations per individual is often limited. Our main result shows that, in the regime where $t \ll N$, the maximum likelihood estimator (MLE) is both statistically minimax optimal and efficiently computable. Precisely, for sufficiently large $N$, the MLE achieves the information theoretic optimal error bound of $\mathcal{O}(\frac{1}{t})$ for $t < c\log{N}$, with regards to the earth mover's distance (between the estimated and true distributions). More generally, in an exponentially large interval of $t$ beyond $c \log{N}$, the MLE achieves the minimax error bound of $\mathcal{O}(\frac{1}{\sqrt{t\log N}})$. In contrast, regardless of how large $N$ is, the naive "plug-in" estimator for this problem only achieves the sub-optimal error of $\Theta(\frac{1}{\sqrt{t}})$.

==> sectionsArxiv/experiments.tex <==
%\begin{figure*}[h!]
\begin{figure}[th!]
  \centering
    %\includegraphics[width=0.95\textwidth]{figures/t10_varyN.pdf}
    \includegraphics[width=0.7\columnwidth]{figuresArxiv/t10_varyN-4.pdf}
    %\vspace{-10pt}
    \caption{Comparing EMD between estimated distribution and truth for varying number of coins (with $t=10$) for various distributions using MLE (blue) and empirical estimate (red).}\label{fig:varyingNt10}
      %\vspace{-15pt}
\end{figure}
%\end{figure*}
%%\vspace{-5pt}
\section{Numerical Experiments}
\label{sec:experiments}
Recall that the MLE (Equation~\ref{eqn:MLEobj}) is a convex optimization problem,
\begin{equation*}
%\vspace{-5pt}
  \hP_{\mle} \in \underset{Q \in \mathcal{D}}{\text{arg max}}\ \sum_{s=0}^t h_s^{\text{obs}} \log{E_Q[h_s]},\nonumber  
\end{equation*}
where $\mathcal{D}$ is the set of all distributions on $[0, 1]$. We discretize the interval $[0, 1]$ into a uniform grid of width $\frac{1}{m}$. Note that as long as the error due to discretization $\mathcal{O}(\frac{1}{m})$ is smaller than the expected error in earth mover's distance (EMD), we will not be losing much numerically. Unless otherwise specified, we use grid length of $m = 1000$. The discretized set $\hat{\mathcal{D}}$ can then be written as $\hat{\mathcal{D}}_m := \left\{ q \in \mathbb{R}^{m+1}: q \geq 0, \one^\top q = 1 \ \right\}$.
We then solve the MLE which is convex on this discrete convex set using cvx~\cite{cvx, grant2008} for Matlab\textsuperscript{\textregistered}.%\\
\iffalse
\begin{IEEEeqnarray}{rCl}
%\vspace{-5pt}
\hP_{\mle}^{(m)} &\in& \underset{Q \in \hat{\mathcal{D}}_m}{\text{arg max}}\ \sum_{s=0}^t h_s^{\text{obs}} \log{E_Q[h_s]},\nonumber
\end{IEEEeqnarray}
\fi
%\begin{figure*}[h!]
\begin{figure}[th!]
  \centering
  %%\vspace{-5pt}
    %\includegraphics[width=0.95\textwidth]{figures/varyt_N1e6.pdf}\label{fig:varyingt}
    \includegraphics[width=0.7\columnwidth]{figuresArxiv/varyt_N1e6-4.pdf}
    %\vspace{-12pt}
    \caption{Comparing EMD between the estimated distribution and ground truth for varying numbers of tosses, $t$, with $N=10^6$ coins, for various distributions using MLE (blue) and empirical estimate (red).}\label{fig:varyingt}
      %\vspace{-10pt}
\end{figure}
%\end{figure*}
\begin{figure}[th!]
  \centering
   %%\vspace{-10pt}
    \includegraphics[width=0.7\columnwidth]{figuresArxiv/realDataCDFfig-2by2.pdf}
    %\vspace{-10pt}
    \caption{CDF of the estimated distribution (top row), and first $t$ moments (bottom row) for (a) political leaning ($t=8$, $N = 3116$) and (b) flight delay datasets ($t=10$, $N = 25,156$) using MLE (blue), moment matching (TKV17)~\cite{Tian2017} (green) and empirical estimate (red). Observed moments is in black.}\label{fig:realdata}
    %\vspace{-10pt}
\end{figure}
\subsection{Simulations on synthetic data:}
%\vspace{-5pt}
We demonstrate the performance of the MLE on synthetic datasets where we know the ground truth.
We consider 4 distributions, (1) single spike at $0.5$, (2) mixture of $3$ spikes of equal mass at $0.25, 0.5$ and $0.75$, (3) truncated Gaussian on $[0, 1]$ with mean $0.5$ and variance $0.1$ and (4) uniform distribution on $[0, 1]$.
\begin{itemize}[leftmargin=*]
    \item \textbf{Varying $t$:} In the first set of experiments we consider the vary $t$ regime where $t = \mathcal{O}\left(\log{N}\right)$. With the population size $N = 1e6$, we vary $t$ from $2$ to $12$. We run MLE, moment matching estimator and empirical estimator. Figure~\ref{fig:smalltN1e6} shows the earth mover's distance (EMD) of the estimates from the true distribution as a function of $t$.

\item  \textbf{Varying $N$:} For $t = 10$, we vary the population size $N$ from $10$ to $10^8$ in multiples of $10$. Figure~\ref{fig:varyingNt10} shows the comparison of performance of the MLE and empirical estimator in EMD. As $N$ increases, the second term in EMD which depends on $N$ decreases. We note that the error in EMD for MLE is much lower than that for empirical distribution when $t \ll N$ as predicted by our analysis.

\item \textbf{Large span of $t$:} For $N = 10^6$ coins, we vary the number of tosses $t$ from $2$ to $10$ in steps of two and then $t = [50, 100, 500, 1000]$ to illustrate the performance of the MLE as $t$ varies widely. Figure~\ref{fig:varyingt} shows the comparison of performance of the MLE and empirical estimator in EMD for various distributions.%\\
\end{itemize}
\subsection{Experiments on real datasets}
%\textbf{Experiments on real datasets:}\\
We ran the MLE on two real datasets used in~\cite{Tian2017}:
\begin{enumerate}
    \item A dataset on \emph{political leanings} of counties in the US with data on whether a county leaned Democratic or Republican for $N=3116$ counties in $t = 8$ presidential elections from $1976$ to $2004$. Here, each county $i$ is assumed to have a true probability $p_i$ with which the county leans Republican in a given election (assuming the independence of counties and elections). 
    \item A dataset of \emph{delays of flights} with $N = 25,156$ flights. Each flight is assumed to have an intrinsic probability $p_i$ of being delayed more than $15$ minutes.
\end{enumerate}
Figure~\ref{fig:realdata} shows the CDF output by MLE, moment matching~\cite{Tian2017} and empirical estimators on these datasets. We note that the observed fingerprints often lie outside the set of valid fingerprints (see Remark~\ref{remark:MLEGeometry}), and hence the solution to the MLE is the projection on the surface. Thus, the MLE tends to give sparser solutions. While the CDF output by the MLE and moment matching qualitatively look very different, their first $t$ moments match and fit the observed first $t$ moments extremely well (bottom row of Figure~\ref{fig:realdata}). Without any side information to enforce constraints like smoothness, it is not possible to pick one over the other with sparse observations. %In contrast, the empirical estimate fits the observed moments poorly. 
%\todo[inline, color=blue!20]{Elaborate a bit about the sparse vs smooth solutions. MLE solution is on the boundary... MLE matches the observed moments as well as finger prints. Moment matches the fingerprint a bit worse.}

